Review of Extreme Multilabel Classification

Extreme multi-label classification or XMLC, is an active area of interest in machine learning. Compared to traditional multi-label classification, here the number of labels is extremely large, hence, the name extreme multi-label classification. Using classical one-versus-all classification does not scale in this case due to large number of labels; the same is true for any other classifier. Embedding labels and features into a lower-dimensional space is a common first step in many XMLC methods. Moreover, other issues include existence of head and tail labels, where tail labels are those that occur in a relatively small number of samples. The existence of tail labels creates issues during embedding. This area has invited application of wide range of approaches ranging from bit compression motivated from compressed sensing, tree based embeddings, deep learning based latent space embedding including using attention weights, linear algebra based embeddings such as SVD, clustering, hashing, to name a few. The community has come up with a useful set of metrics to identify correctly the prediction for head or tail labels.

==> DeepLearning/all-deep-learning.tex <==
\paragraph{}
Deep Learning as a field has exploded in the recent past and has started to become a dominating method in most machine learning problems, where there is a large amount of available data. In extreme multi label classification, deep learning did not make an advent until much later due to several possible reasons. Firstly, the output space being extremely large implies the requirement of very large models. Secondly, the very large tail-label distribution implies that a large set of labels have very little training data available, hindering the ability for deep learning models to learn enough to predict these labels correctly. For example, in the Wiki-500K dataset \cite{Bhatia16}, 98\% of labels have less than 100 training instances. Thus, efforts to use Deep Learning in the field were not as successful and linear algebra and tree based methods dominated.

However, Deep Learning was very successful in extracting context dependent information from the raw text due to the highly non-linear nature of learning. With this ability to obtain highly representative embeddings from the text, the usage of bag-of-word models in XML was contested by deep-learning based methods. 

% \subsubsection{Deep Learning for Extreme Multi-label Text Classification (XML-CNN)}

\paragraph{}

The paper \cite{liu2017deep} was the first to try out application of Deep Learning in XML, using a family of CNN's. This followed the success of deep learning in multi-class text classification problems by methods like FastText \cite{joulin2016bag}, CNN-Kim \cite{chen2015convolutional} and Bow-CNN \cite{liu2017deep}. These methods inspire this new method XML-CNN which applies similar concepts to obtain an extreme multi-label classifier. 

CNN-Kim \cite{chen2015convolutional} creates a document embedding from concatenation of word embeddings. $t$ CNN filters are applied to obtain a $t$ dimensional vector which is passed to a soft-max layer after max pooling. Bow-CNN \cite{liu2017deep} creates a $V$ dimensional vector for each region of the text, where $V$ is the vocabulary size, indicating whether each word is present in the region. It also uses dynamic max pooling for better results. XML-CNN combines these ideas and proposes the following architecture - various CNN filters similar to CNN-Kim, dynamic max pooling similar to Bow-CNN, a bottleneck fully connected layer, and binary cross entropy loss over a sigmoid output layer. 

\paragraph{}
Let $e_i \in R^k$ be the word embedding of the $i-$th word of the document, then $e_{i:j} \in R^{k(j-i+1)}$ is the concatenation of embeddings for a region of the document. A convolution filter $v$ is applied to a region of $h$ words to obtain $c_i = g_c(v^Te_{i:i+h-i})$ which is a new feature, where $g_c$ is a non-linear activation. $t$ filters like this are used with varying $h$ to obtain a a set of new features. 

\paragraph{}
Dynamic Max pooling is then used on these newly obtained features $c$. The usual max pooling basically takes the maximum over the entire feature vector to obtain a single value. However, this value does not sufficiently represent the entire document well. Thus, a max-over-time pooling function is used to aggregate the vector into a smaller vector by taking max over smaller segments of the initial vector. Thus, pooling function $P$ is given by 
\begin{align*}
P(c) = \left[\max \left(c_{1:\frac{m}{p}} \right), \, \dots , \, \max \left(c_{m-\frac{m}{p}+1:m} \right) \right] \in \R^p.
\end{align*}
This pooling function can accumulate more information from different sections of the document. These poolings from different filters are then concatenated into a new vector.

\paragraph{}
The output of the pooling layer is now fed into a fully connected layer with fewer number of neurons, also called a bottleneck layer. This bottleneck layer has two advantages. Firstly, it reduces the number of parameters from $pt \times L$ to $h \times (pt + L)$ where $L$ is the number of labels, $t$ is the number of filters, $p$ is the pooling layer hyperparameter and $h$ is the number of hidden layers in the bottleneck layer. This allows the model to fit in memory as L is often large. Secondly, another non-linearity after the bottleneck layer leads to a better model. Thirdly, this encourages the learning of a more compact representation of the data.


\begin{figure}[t!]
%\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.4]{Images_K/XML_CNN.drawio.png}
    \caption{\label{fig:CnnXML} The XML-CNN model }
\end{figure}

Finally, the output of the bottleneck layer is passed through another fully connected layer with output size $L$. The binary cross entropy loss is observed to work the best used for this method. 

The ablation studies performed in the paper show that BCE loss, bottleneck layer, and dynamic max pooling each contribute to the improvement of the model. Though XML-CNN was slower than the tree based methods, it clearly outperformed them in terms of performance. It also performed better than linear algebra based methods, showing the potential deep learning held for the XML field.


% \subsubsection{AttentionXML: Label Tree-based Attention-Aware Deep Model for High-Performance Extreme Multi-Label Text Classification (NIPS'19)}

\paragraph{}

However, XML-CNN was unable to capture the most relevant parts of the input text to each label, because the same text representation is given for all the labels. Sequence to Sequence based methods like MLC2Seq \cite{MLC2Seq} were also not suited for the task since the underlying assumption that labels are predicted sequentially is not reasonable in extreme classification. \cite{you2019attentionxml} proposed \textbf{AttentionXML}, which used a BiLSTM (bidirectional long short-term memory) to capture long-distance dependency among words and a multi-label attention to capture the most relevant parts of texts for each label. Since application of attention to train on each label with the full dataset is not possible for large datasets, there must be a method for training on only the most relevant samples for each label. For this, AttentionXML uses a shallow and wide Probabilistic Label Tree (PLT) built on the labels.

\paragraph{}
The first step is to create the PLT, which is be done by hierarchical clustering algorithm followed by a compression algorithm to reduce depth. This step is similar to that of Parabel \cite{prabhu2018parabel} where we create a label tree, but here the tree is constructed to be wide and shallow. In effect, the label tree resembles that of Bonsai \cite{khandagale2020bonsai}. The reason for creation of a wide tree instead of a deep one is to prevent error propagation through the levels. The leaves correspond to an original label while the internal nodes correspond to meta or pseudo labels. Each node predicts $P(z_n | z_{Pa(n)}=1, x)$, ie the probability that label or pseudo-label $n$ is present, given that parent of $n$ is present. Thus, the marginal probability for each label being present is given by the product of probabilities in its path in the PLT i.e.,
\begin{align*}
    P(z_n =1 \mid x) = \Pi_{i \in \text{Path}(n)} P(z_i \mid z_{Pa(i)}=1, x).
\end{align*}
The value of the marginal probabilities is predicted by the attention based deep learning network. As depicted in \ref{fig:AttnXML}, the architecture consists of a bidirectional LSTM which finds embeddings for the words and then followed by a 2-layer fully connected neural network which finally predicts the probability that the current label is active given the input. There is one block of such network per layer of the PLT. 

\paragraph{}
The input to the fully connected layers is given by using a attention based mechanism which can find if a word embedding is relevant to the label. Finally, the parameters of the fully connected layers are shared among the different labels in each layer, as they perform the same function. This also largely helps reduce model size. Further, to reduce training cost, the model weights of each layer is initialized with the weights of the previous layer.

%\small
\begin{figure}[t!]
%\begin{figure}[ht] 
    \centering
    \includegraphics[scale=0.3]{Images_K/AttentionXML.drawio.png}
    \caption{\label{fig:AttnXML} An Illustration of Attention Aware Deep Model in AttentionXML }
\end{figure}

\paragraph{}
It is to be noted that even if this network is directly used, the training time will be infeasible as each label would have to train on each sample. However, we do not need to train on every sample for a particular label. Hence, only the samples which contain the label and a few more negative samples are used for training.

\paragraph{}
AttentionXML outperforms XML-CNN and most other methods in terms of P@1 scores. Further, the good PSP scores show that AttentionXML performs well on tail labels as well. The utility of multi-head attention is proven in the ablation study. However, AttentionXML is not easy to train as the training and prediction times are much larger compared to other methods and hence does not scale well to larger datasets.

% \paragraph{Detailed Discussion}
% In this paper probabilistic label tree is constructed similar to that of the parabel. Label representations have to be computed and then using this label representations the labels are recursively partitioned into two balanced clusters at each node. In the parabel recursive partitioning of the nodes is stopped when there are no more than 100 or 200 labels. But here that number is very less, hence the obtained probabilistic label tree is deep. Then some levels of the deep tree are pruned, so that the tree becomes a shallow and k-ary tree. 

% Authors in this paper claimed that because of the deep tree structure, the errors are accumulated along the tree. Hence pruned the tree this way to obtain a shallow tree. Also in this way there are few labels at each node, thus lessening the chance of tail and head labels partitioned into the same leaf node.Another observation is that the classifiers at each node doesn't have enough representational power to model. Hence in this paper a DeepNet with attention is used at each level.  

% The input to this network is the set of words ${ ( x_i )_{1}^T} $ where each word $ x_i \in \R^{300} $ is a word embedding. In this paper the Glove word embedding is used. The BiLSTM consists of the 


%\newpage
% \subsubsection{DeepXML: Scalable \& Accurate Deep Extreme Classification for Matching User Queries to Advertiser Bid Phrases (ICLR'20)}

% DEEPXML splits training of head and tails labels separately. It tries to increase the accuracy of their model by 

% (a) Learning word embeddings on head labels and transferring them through a novel residual connection to data impoverished tail labels.

% (b) Increasing the amount of negative training data available by extending state-of-the-art negative sampling techniques.

% (c) Re-ranking the set of predicted labels to eliminate the hardest negatives for the original classifier.

% \textbf{Matching queries to bid phrases :} Web search engines allow ads to be served for not just queries bidded on directly by advertisers, referred to as bid phrases, but also for related queries with matching intent. Thus matching a query that was just entered by the user to the relevant subset of millions of advertiser bid phrases in milliseconds is an important research application.

% For example, given the user query - \say{What is diabetes type 2} as input. DeepXML predicts that ads corresponding to the bid phrases - \say{What is type 2 diabetes mellitus}, \say{diabetes type 2 definition}, \say{do I have type 2 diabetes}, etc. could be relevant to the user. 

% \textbf{SOTA extreme classifiers: } Learning extreme classifiers based on the bag-of-words (BOW) features (Parabel) and pretrained embeddings (Slice) are highly scalable but inaccurate for documets having only 3 or 4 words. Even XML-CNN and AttentionXML's architectures have not been specialised for short text documents.


% \paragraph{Observations \& Contributions of the Authors}
% \begin{itemize}
%     \item \textbf{Observation: } XML-CNN\cite{XML_CNN} cannot capture the most relevant parts of the input text to each label, because the same text representation is given for all the labels. Sequence to Sequence based methods like MLC2Seq\cite{MLC2Seq} are not suited for the task since the underlying assumption that labels are predicted sequentially is not reasonable in extreme classification.
    
%     \textbf{Contribution: } Proposed a BiLSTM(bidirectional long short-term memory) to capture long-distance dependency among words and a multi-label attention to capture the most relevant parts of texts to each label
    
%     \item \textbf{Observation: } A tree based method Parabel has issues. The height of the tree and the cluster size in Parabel model may deteriorate its performance. In deep trees errors may be accumulated and progated along the tree while training. Because of large cluster size tail labels may end up in cluster with dissimilar labels leading to poor accuracy.
    
%     \textbf{Contribution: } In these papers, authors pruned the probabilistic label tree (PLT) used in the Parabel so that the resulting tree is short and wide ( many leaves i.e., a small cluster size).
    
% \end{itemize}

% \paragraph{Architecture}

% AttentionXML model consists of 
% \begin{itemize}
%     \item A shallow and wide PLT.
%     \item Deepnet with BiLSTM and Attention for each level of PLT.
% \end{itemize}
% \small
% \begin{figure}[htb]
% %\begin{figure}[ht]
%     \centering
%     \includegraphics[scale=0.5]{Images_K/AttnXML.png}
%     \caption{\label{fig:AttnXML} An Illustration of Attention Aware Deep Model in AttentionXML }
% \end{figure}

% \paragraph{Detailed Discussion}
% In this paper probabilistic label tree is constructed similar to that of the parabel. Label representations have to be computed and then using this label representations the labels are recursively partitioned into two balanced clusters at each node. In the parabel recursive partitioning of the nodes is stopped when there are no more than 100 or 200 labels. But here that number is very less, hence the obtained probabilistic label tree is deep. Then some levels of the deep tree are pruned, so that the tree becomes a shallow and k-ary tree. 

% Authors in this paper claimed that because of the deep tree structure, the errors are accumulated along the tree. Hence pruned the tree this way to obtain a shallow tree. Also in this way there are few labels at each node, thus lessening the chance of tail and head labels partitioned into the same leaf node.Another observation is that the classifiers at each node doesn't have enough representational power to model. Hence in this paper a DeepNet with attention is used at each level.  

% The input to this network is the set of words ${ ( x_i )_{1}^T} $ where each word $ x_i \in \R^{300} $ is a word embedding. In this paper the Glove word embedding is used. The BiLSTM consists of the 
% %\newpage
% \subsubsection{DeepXML: Scalable \& Accurate Deep Extreme Classification for Matching User Queries to Advertiser Bid Phrases (ICLR'20)}

% DEEPXML splits training of head and tails labels separately. It tries to increase the accuracy of their model by 

% (a) Learning word embeddings on head labels and transferring them through a novel residual connection to data impoverished tail labels.

% (b) Increasing the amount of negative training data available by extending state-of-the-art negative sampling techniques.

% (c) Re-ranking the set of predicted labels to eliminate the hardest negatives for the original classifier.

% \textbf{Matching queries to bid phrases :} Web search engines allow ads to be served for not just queries bidded on directly by advertisers, referred to as bid phrases, but also for related queries with matching intent. Thus matching a query that was just entered by the user to the relevant subset of millions of advertiser bid phrases in milliseconds is an important research application.

% For example, given the user query - \say{What is diabetes type 2} as input. DeepXML predicts that ads corresponding to the bid phrases - \say{What is type 2 diabetes mellitus}, \say{diabetes type 2 definition}, \say{do I have type 2 diabetes}, etc. could be relevant to the user. 

% \textbf{SOTA extreme classifiers: } Learning extreme classifiers based on the bag-of-words (BOW) features (Parabel) and pretrained embeddings (Slice) are highly scalable but inaccurate for documets having only 3 or 4 words. Even XML-CNN and AttentionXML's architectures have not been specialised for short text documents.





% \subsubsection{Taming Pretrained Transformers for Extreme Multi-label Text Classification (XTransformer)}

\paragraph{}

Despite the usage of attention by AttentionXML, a direct attempt at using the pretrained transformers for XML was not yet made. The transfer learning of pretrained transformers for this task could be the solution to the large training times required by AttentionXML. \cite{chang2020taming} made the first attempt at using pretrained transformers for the XML task in the model \textbf{XTransformer}. Transformers like BERT \cite{devlin2018bert}, RoBERTa \cite{liu2019roberta}, and XLNet \cite{yang2019xlnet} are highly successful in the NLP domain where they outperformed most other methods on tasks like question answering, POS tagging, and sentence classification due to their ability to generate contextual embeddings for words and sentences which are applicable to downstream tasks. However, application of these models for the XML problem was not so straightforward even though XML is primarily a text classification problem. 

\paragraph{}
The difficulty was because of the large number of labels and the output space sparsity. Many of the labels do not have enough samples to be able to be able to train large deep neural networks and hence direct application of pretrained transformers led to bad results and memory issues. Xtransformer handles this by reducing the larger problem into smaller subproblems, like in tree based methods, and then training the transformers to predict in this smaller problem. Each of the subproblems are eventually solved to get the final predictions.

\paragraph{}
More concretely, the XTransformer model consists of three parts or modules. The first module is called Semantic Label Indexing, which is responsible for the division of the larger problem into smaller subproblems. For this, a clustering of the labels is performed, creating $K$ clusters where $K \ll L$. The clusters are created by finding a label to cluster assignment matrix $C \in \{0,1\}^{L\times K}$ where $C_{lk} = 1$ if label $l$ belongs to cluster $k$. This matrix can be created by using hierarchical clustering algorithms and the clusters are represented based on the mean of transformer embeddings of the label text for the labels present in the cluster. 

\paragraph{}
These clusters are then used as meta-labels for the problem of fine tuning the transformer models in the second module called the Neural Matcher. Since the number of meta-labels is much smaller, the  label sparsity issue due to tail labels is avoided. The transformers are trained to map from instances to the relevant clusters. Embeddings $\phi(x)$ are thus trained for each instance $x$. 

\paragraph{}
In the third module after the matching step, a small subset of label clusters is selected for each instance from which we are required to find a relevance score of each label. For performing this final step which is crucial to prediction, a one-vs-all classifier is trained for each label. The instances on which each label trains must be limited in number to allow efficient training. Techniques like picking teacher-forcing negatives (for each label $l$, picking only the instances instances with label $l$ or with any of the labels in the same cluster as label $l$) allow picking only a small subset of ``hard" instances. 


\begin{figure}[t!]
%\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.36]{Images_K/XTransformer.drawio.png}
    \caption{\label{fig:AttnXML} The XTransfomer method }
\end{figure}

\paragraph{}
During prediction, a subset of clusters are selected by the Matcher. All the labels selected from each of the clusters are then passed the test instance to which each one-vs-all classifier gives a relevance score to decide if the label is relevant to the instance, based on which the label ranking is done. XTransformer is successfully able to perform well on all datasets and was only outperformed by AttentionXML on some datasets at the time.

\paragraph{}
Some other successful methods which attempt to fine tune transformers have been recently proposed such as APLC-XLNet, \cite{ye2020pretrained} which uses transfer learning of the popular transformer model XLNet \cite{yang2019xlnet}. As with previous methods, performing this directly is not possible, hence this methods uses Adaptive Probabilistic Label Clusters, which attempts a clustering based on separating the head and tail clusters, and then assigning head cluster as the root of a tree and tail clusters as leaves. 

\paragraph{}
Another method which uses transformers to perform extreme classification is LightXML \cite{jiang2021lightxml}. This paper points out that methods like AttentionXML and XTransformer suffer from static negative sampling, which highly reduces the ability of the model. The main advantage of LightXML over other methods using static negative sampling is that the model does not overfit to specific negative samples. LightXML performs dynamic negative sampling by using a generator-discriminator like method in which the label recalling is performed by a module (generator) and the label ranking is done by another module. This procedure allows each module to try and improve its own objective while enhancing the other, thus leading to better performance overall. 


\paragraph{}
The transformer-based approaches like X-Transformer \cite{chang2020taming} above and LightXML \cite{jiang2021lightxml} achieve state-of-the-art XMC results by clustering labels to reduce computational complexity. However, they still face significant memory and training time issues with larger label spaces.\\
XR-Transformer \cite{zhang2021fast}, addresses these computational challenges by leveraging recursive shortlisting and hierarchical label trees (HLTs)\cite{10.1145/3178876.3185998}. XR-Transformer recursively fine-tunes pre-trained transformers, on progressively smaller label spaces, ultimately reducing the computational burden. This recursive process ensures that for any input, the number of candidate labels considered during training and inference is \(O(B)\), and the total number of labels is \(O(B \log_{B}(L))\), where \(B\) is the cluster size and \(L\) is the labels.\\
The key steps in XR-Transformer are as follows:
\begin{enumerate}
\item Labels are recursively clustered using balanced $k$-means, forming a hierarchical label tree (HLT). Label features \( Z \in \mathbb{R}^{L \times \hat{d}} \) are constructed using text vectorizers or Positive Instance Feature Aggregation (PIFA),
    $$
Z_{\ell}=\frac{{v}_{\ell}}{\left\|{v}_{\ell}\right\|} ; \text { where } {v}_{\ell}=\sum_{i: y_{i, \ell}=1} \Phi\left({x}_i\right), \forall \ell \in[L]
$$ 
where \( \Phi : \mathcal{D} \to \mathbb{R}^d \) is the text vectorizer.

\item Coarse label vectors are obtained through max-pooling, creating a series of coarse-to-fine learning signals. To mitigate information loss when merging positive labels, XR-Transformer uses recursively constructed relevance matrices, which assign non-negative importance weights to each instance and label cluster.
\item Instead of training on the entire label space, it shortlists labels based on the relevance scores and the top-$k$ relevant clusters from the parent layer. This shortlisting approach, combined with multi-resolution learning, defines a series of learning objectives that progressively refine the model's ability to predict relevant labels efficiently.
\end{enumerate}

\paragraph{}
Another notable feature of XR-Transformer is its combination of statistical text features (such as TFIDF) and semantic transformer embeddings. This dual representation mitigates the information loss associated with text truncation in transformers and leverages the strengths of both statistical and deep learning approaches.\\
Empirical results show XR-Transformer significantly improves training efficiency and performance on six public XMC benchmarks datasets(Eurlex-4K, Wiki10-31K,
AmazonCat-13K, Wiki-500K, Amazon-670K, Amazon-3M). On the Amazon-3M dataset, it increased Precision@1 from 51.20\% to 54.04\% and reduced training time from 23 days to 29 hours, highlighting its scalability and efficiency without sacrificing accuracy.


\paragraph{}
The paper  \cite{chien2023pina} presents Predicted Instance Neighborhood Aggregation (PINA), the primary focus is on leveraging side information, such as label metadata and instance correlation signals, to improve the performance of XMC models. By drawing parallels between XMC and neighborhood prediction problems in graph learning \cite{chien2022node}, the authors propose a method that augments traditional XMC models, such as XR-Transformers \cite{zhang2021fast}, with additional contextual information to improve performance. They utilize this connection to leverage advanced techniques from graph convolutional networks \cite{hamilton2018inductive} and neighborhood aggregation, which have been proven effective in various graph-based tasks.\\
The pretraining task integrates both instance and label text as inputs. This task constructs a biadjacency matrix to represent the multi-label relationships in an undirected manner, allowing the model to consider label text directly during pretraining. This is a significant departure from traditional XMC models(\cite{you2019attentionxml},\cite{zhang2021fast}) that typically ignore label text in their training processes.\\
PINA operates in two stages:
\begin{itemize}
    \item \textbf{Pretraining Phase: }Here, the model learns a neighbor predictor using both instance and label text, both instance and label text are used to construct a pretraining XMC problem. This phase results in a text vectorizer capable of generating numerical features for both instances and labels.

    \item \textbf{Augmentation Phase:} During the augmentation phase, the pretrained neighbor predictor generates neighborhood predictions for both training and test instances. The top-$K$ predicted neighbors are used to aggregate features, enhancing the original instance features with additional contextual information from the neighbors.
\end{itemize}
On the largest dataset, LF-AmazonTitles-1.3M, PINA achieves approximately a 5\% gain in accuracy compared to standard XR-Transformers. This substantial improvement underscores the effectiveness of incorporating side information and leveraging neighborhood aggregation in handling large-scale XMC problems.


% \subsubsection{DeepXML: A Deep Extreme Multi-Label Learning Framework Applied to Short Text Documents (ASTEC)}

\paragraph{}

A general trend can be observed from papers like AttentionXML and XTransformer, where deep learning methods are not directly applied to the problem due to scalability issues. Instead, the deep learning model is applied to a smaller subproblem to obtain intermediate features which can be further used in the problem. Also, negative sampling is generally used for training the final model as training on all samples is not feasible. \cite{dahiya2021deepxml} comes up with a general framework for applying deep learning methods to XML called DeepXML. Consequently, they propose a new method called ASTEC using the existing method which achieves a new state of the art for some datasets in the domain. 

\paragraph{}
The paper defines DeepXML to be a framework with four modules. Each module is designed to be fairly of low complexity, allowing the entire method to scale to large datasets easily. Not all the methods need to have each of the modules depending on the utility, and the module algorithm can be switched to another algorithm easily without affecting the entire method.

\paragraph{}
The first module of the framework is for training intermediate representations for the features $Z^0$. Here, $Z^0$ should be as close as possible to the final representation of the features $Z$ which would be the feature representations if the entire problem was optimized directly.  Since features cannot be trained on the entire problem, a surrogate label selection procedure is followed to ensure that the problem is tractable. Some examples of surrogate label selection procedures could be label subset selection, label clustering or or label projection into a smaller space.

\paragraph{}
The second module of DeepXML is the label shortlisting or the negative sampling step, where for each sample, we select the most confusing of the "hardest" labels. We select $N_i \subseteq [L]$ for each sample $i$ such that $|N_i| = O(\log L)$ and these labels are most likely to be predicted as positive labels for the samples. This negative sampling is done based on the intermediate features learnt in the first module and any method can be used for this procedure such as graphs, trees, clustering or hashing.

\paragraph{}
The third module is based on transfer learning to obtain the final feature representations from the initial feature representations learnt in the first module. The parameters can be re-trained from the first module, but it must be ensured that the final feature representation $Z$ should not be too far from the initial representation.

\paragraph{}
In the fourth module, the final classifier is learnt. This classifier uses the feature representation from the third module and the negative samples from the second module. Since the number of instances for each label is not excessive due to the negative sampling, the model training time is limited. The third and fourth modules can be combined as required.

\begin{figure}[t!]
%\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.35]{Images_K/DeepXML.drawio.png}
    \caption{\label{fig:DeepXML} Overview of the DeepXML Framework}
\end{figure}

\paragraph{}
In the paper \cite{dahiya2021deepxml}, the method ASTEC is proposed which uses the DeepXML framework. For the first module, it uses a tree based clustering method to obtain the surrogate labels for training intermediate features. For the second module, an Approximate Nearest Neighbor Search (ANNS) data structure is used for shortlisting. Modules 3 and 4 are trained together where the transfer learning is done by a simple transfer matrix, while the final classifiers are simple one-vs-all classifiers. 

\paragraph{}
More methods using this framework have also been proposed and several existing ones, such as XTransformer can can be formulated to fit into this framework. \cite{mittal2021decaf} proposes a method DECAF using this framework which incorporates the label metadata. \cite{mittal2021eclare} proposes ECLARE which utilizes label to label correlation as well as label text to give a new method following the DeepXML framework. GalaXC \cite{saini2021galaxc} is another method in this framework which uses graph neural networks on the combined document label space.

\paragraph{}
Recent advances have been made in the field by using the label features in addition to the instance features. Since in many of the XML datasets, the labels are also entities with some text information. This allows using the label text for learning better models. Different methods try to utilize the label features in different ways. For example, DECAF \cite{mittal2021decaf} directly incorporates label text into the classification procedure by embedding the instances and labels separately and then using a ranker to predict which label embedding is most relevant to the instance.

% Add ECLARE
\paragraph{}
On the other hand, GalaXC \cite{saini2021galaxc} utilizes graph neural networks to learn embeddings jointly over documents and labels. The method uses convolutions of varying size to develop an attention mechanism for learning several representations for each node, where each document and label is a node.
% This method is also based on the DeepXML framework.
Multiple hops over the joint label and document graph allow collection of information over related labels, other documents with these labels and so on. This is used for shortlisting and then prediction is finally made by using the label attention mechanism. 
ECLARE \cite{mittal2021eclare} also uses a similar method by accommodating for label metadata and label correlations. 

\paragraph{}
SiameseXML \cite{dahiya2021siamesexml} also uses label features, but it aims to learn joint embeddings for the labels and features by using the concept of Siamese Networks \cite{chen2020simple}, \cite{schroff2015facenet} where a triplet or contrastive loss is used with a hard negative mining procedure. The main goal is to learn common embeddings for instances and labels where instances are close to the respective positive labels and far from the other negative labels. This concept is adapted to the extreme classification scenario by using the DeepXML framework.

\paragraph{}
The paper \cite{dahiya2022ngame} suggests another method NGAME which uses Siamese Networks for extreme classification. A common method of using Siamese Networks is using minibatches. The set of candidate labels contains all the labels which appear in at least one of the other instances in the minibatch. The minibatch size, if constructed independently, cannot be too large as the set of labels would be to big. This leads to slower training. NGAME strategically constructs the mini-batches such that the samples are close, thus leading to informative negative samples as compared to random samples. This leads to better convergence and faster training.

% Recently, there has been progress in 






% \paragraph{DEEPXML approach.} In the DeepXML approach,

% \begin{itemize}
%   \item Partitioning all $L$ labels into a small set of head labels, with cardinality less than $0.1L$, containing the most frequently occurring labels and a large set of tail labels containing everything else.
  
%   \item DeepXML first represented a document by the tf-idf weighted linear combination of its word-vector embeddings.
  
%   \item The word-vector embeddings of the training documents were learnt on the head labels where there was enough data available to learn a good quality representation of the vocabulary. Accuracy was further boosted by the introduction of a novel residual connection to fine-tune the document representation for head labels.
  
%   \item The word-vector embeddings were then transferred to the tail network where there wasn't enough data available to train them from scratch.
 
%   \item Once the word vector embeddings have been trained on the head, they are frozen and transferred to the tail where only the residual block is fine tuned.  
% \end{itemize}

% \paragraph{Architecture and Training}
% \textbf{DeepXML-h: } Model parameters i.e word embeddings, residual block, and fully connected classifier are learnt with binary cross entropy loss and Adam. DeepXML-h can be efficiently trained with a fully connected final layer on a single GPU, as $L_h$ contains only a small subset of labels. Additionally, ANNS structure was trained over label centroids $L_{h}^c$ of head labels. 

% \textbf{DeepXML-t: } Relies on Slice to fine-tune the residual block in the tail network and learn the weights in the full connected output layer for millions of tail labels. Slice achieves this by first representing each label by the unit normalized mean of the feature vectors of the training points tagged with the label. It then learns an ANNS data structure over the label representations to determine the most likely labels for a given data point.

% \small
% \begin{figure}[h]
%     \centering
%      \includegraphics[scale=0.35]{Images_SK/deepxml.png}
    
%     \caption{\label{fig:deepxml}Architecture of DeepXML with DeepXML-h for head labels and DeepXML-t for tail labels. Residualblock is a sequence of linear transformation, Batch Normalization, ReLU and Dropout operations. Here $\bigotimes$ refers to matrix-vector multiplication. Gradients are not propagated through dotted lines.   }
    
% \end{figure}

% \textbf{Prediction}\\
% Initially classifier scores and ANNS scores from both DeepXML-h and DeepXML-t are merged in a single vector $\hat{y}$. $\hat{y}_{clf-h}$ is the classifier score from DeepXML-h and $\hat{y}_{anns-h}$ is the cosine similarity from ANNS-h. $ \hat{y} = (1-\beta) * \sigma([\hat{y}_{anns-h};\hat{y}_{anns-t}]) + \beta * \sigma([\hat{y}_{clf-h};\hat{y}_{clf-t}])
% $, where $\sigma$ is a sparse sigmoid function computed only at non-zero entries \& $\beta \in [0,1]$.



The paper \cite{10470392} introduces us to a novel approach MatchXML: a more efficient  text
label matching framework for XMC. Prior work \cite{NEURIPS2021_3bbca1d2},\cite{LightXML}, \cite{DBLP:journals/corr/abs-1905-02331} includes TF-IDF and PIFA \cite{Yu2019} for label embedding generation but these have some limitations as TF-IDF doesn't capture semantic meaning of text corpora due to the ignorance of word order and in PIFA also, we generate label embeddings using TF-IDF features. This paper generates the final text representations by taking the advantage of both sparse TF-IDF features and dense vector features. 

\paragraph{}
Firstly, label2vec is developed to generate dense label embeddings, which are used to construct a Hierarchical Label Tree (HLT) \cite{10.1145/3178876.3185998}. These dense embeddings outperform traditional TF-IDF representations, especially on large datasets, by better capturing semantic information and reducing embedding size significantly. Secondly, MatchXML reformulates the multi-label classification task as a text-label matching problem within mini-batches by pairing each text instance with a subset of relevant and irrelevant labels in each mini-batch. This approach involves fine-tuning the encoder Transformer to distinguish between matching and non-matching text-label pairs using a loss function designed to maximize the similarity between correct text-label pairs and minimize it for incorrect ones. This approach leverages mini-batch training to efficiently learn robust text representations that align closely with the corresponding labels.

\paragraph{}
Additionally, the framework incorporates static sentence embeddings from pre-trained sentence transformers, complementing the sparse TF-IDF features and dense text embeddings fine-tuned from pre-trained transformers. This combination improves the model's ability to handle longer text sequences and enhances overall performance. 

\paragraph{}
An ablation study demonstrates the effectiveness of each component, with label2vec showing superior performance on large datasets and text-label matching outperforming baseline methods in most cases. The integration of static sentence embeddings further boosts performance across various metrics. Empirical evaluations on six benchmark datasets reveal that MatchXML achieves superior classification accuracy and training speed compared to existing methods.  



The existing deep learning based XML methods are optimized for head labels, but this paper mainly focuses on performance of tail labels using deep learning based XML method, BoostXML, enhanced by Gradient Boosting. 
 In BoostXML method, the classifier and the training process is modified to suit the gradient boosting, remaining architecture is similar as other deep learning XML methods \cite{LightXML}, \cite{DBLP:journals/corr/abs-1811-01727}. 

 \paragraph{}
 BoostXML, inspired by \cite{Kang2020Decoupling}, follows a two stage training scheme  where the representation learning stage (i.e., the first stage)
 performs end-to-end network training with regular cross
entropy loss, and classifier adaption stage (i.e., the second
 stage) is conducted with encoder fixed. 
 In the first stage, pretraining step is introduced, in this BoostXML conducts representation learning via the training procedure of AttentionXML, whose instance representation learning module is called the backbone network.

 \paragraph{}
The second stage consist of boosting step and corrective step. In boosting step, gradient boosting $F_t(x)=F_{t-1}(x)+\rho_t f_t(x)$ is used to fit all the residuals of tail labels, here $F_t(x)$ is ensemble of $t$ functions and $\rho_t$ is the weight of $t^{\text{th}}$ function and it will take only shared binary classifier (here shared classifier refers to same classifier used to classify multiple labels) as the base learner. In BoostXML's Boosting Step, each base learner (an MLP) is trained from scratch to fit residual errors. Label-specific representations are obtained via a shared encoder, and the objective function is the mean squared error (MSE). To ensure weak learners, MLPs are trained with few epochs and random initialization. Both first-order and second-order gradients are used to enhance the model's focus on misclassified tail labels, improving classification performance through amplified residuals.

\paragraph{}
The Corrective Step in BoostXML updates the entire network, including the encoder and all previous weak learners, through back-propagation after training each new weak learner. This step uses Binary Cross Entropy (BCE) as the objective function, ensuring better representation learning and adaptation of weak classifiers. It helps avoid local minima and improves overall model performance by allowing dynamic adjustment of the boosting rate.

\paragraph{}
 BoostXML is evaluated on five benchmark datasets ( EUR-Lex, Wiki10-31K, AmazonCat-13K,  Wiki-500K and
 Amazon-3M)  to compare its performance with state-of-the-art XML methods. Deep learning based baseline methods used here are AttentionXML by \cite{AttentionXML},  LightXML by \cite{LightXML} and in non deep learning baseline methods AnnexML by \cite{AnnexML}, FastXML by \cite{FastXML}, PfastreXML by \cite{PfastreXML} are used. BoostXML outperrforms the SOTA methods on most of the baseline methods, particularly on tail labels without compromising the performance on the head labels.



For long-tail distribution a natural solution comes in mind is data augmentation technique to compensate the scarce data \cite{10.1007/978-3-031-05933-9_11} \cite{10.1609/aaai.v37i9.26259}. There are some existing works \cite{zhou-etal-2022-flipda}, \cite{wang-etal-2022-promda} which resort to applying Pretrained Language Models (PLM) for data augmentation in low resource setting, but these approaches struggle in multi-label scenarios due to label co-occurrence \cite{DBLP:journals/corr/abs-2007-09654}. The paper \cite{10446315} introduces a novel approach, Extreme Data Augmentation (XDA), that addresses these challenges and alleviate the low quality and long-tailed problem of augmented samples by employing three key mechanisms: \textit{Prompt, Filter} and \textit{Mask}.

\paragraph{}
 Motivated by \cite{lester-etal-2021-power}, \cite{wang-etal-2022-promda}, employ the softprompt technique for fine tuning by adding a sequence of trainable vectors $ P^j=\{p_1^j,...,p_k^j\}$ at each transformer layer
  and update the parameters of soft-prompt only while keeping the all other PLM parameters fixed.  The pre-trained model $f_0$
  employs the original training set to learn a mapping from input texts 
$x$ to feature vectors, using a text encoder $\phi$ and classifier parameters 
$w_l$, with binary cross entropy (BCE) as the loss function,
 \begin{equation}
        L_{\text{BCE}} = - \left( y \log(\sigma(f(x, l))) + (1 - y) \log(1 - \sigma(f(x, l))) \right)
    \end{equation}
    providing essential feedback signals for the sample filtering process. In filtering, check the semantic difference between an augmented sample $x_i^j$ and its original corresponding sample $x_i$, by using KL-divergence, the divergence score $S_{\text{Div}}^{i,j}$ of augmented sample $x_i^j$ is given by
  \[S_{\text{Div}}^{i,j}=D_{\text{KL}}(p(\sigma(W_0^T \phi_0(x_i^j))) \, \| \, p(y_i)), \]
  which gives us the diversity between these two distributions, here $\phi_0$ is the text encoder that maps $x$ to a feature vector, $W_0$ is the weight of the trainable classifier, and for augmented process we can consider high diversity between augmented samples. We also need to check the consistency score, because low quality samples will lead to label drift \cite{zhou-etal-2022-flipda},\cite{kamalloo-etal-2022-chosen}. The consistency score $S_{Con}^{i,j}$ of augmented sample $x_i^j$ is given by \[ S_{\text{Con}}^{i,j} =\frac{1}{k_i}| \text{Top}_{k_i}(f_0(x_i^j)) \cap \text{Top}_{k_i}(f_0(x_i))|,\]
  
  where $f_0$ denotes the pretrained model.

  \paragraph{}
  By jointly considering $S_{\text{Div}}^{i,j}$ and $ S_{\text{Con}}^{i,j}$, high quality samples are selected with balanced diversity and consistency.
Now in the final step, directly using augmented samples might exacerbate the long-tailed problem, to address this issue divide the head and tail labels by some threshold and during training, augmented sample-label pairs associated with head-labels are masked. The loss function incorporates a mask indicator $m=\{m_l \}_{l=1}^L$, ensuring a balanced focus on tail-labels, \begin{equation*}
            L_{\text{Aug}} = -\sum_{l=1}^L m_l \left[ y_l \log (\sigma(f_0(x, l))) + (1 - y_l) \log (1 - \sigma(f_0(x, l))) \right]
        \end{equation*}
        where $m_l = 0$ if $l$ is a head-label and $m_l = 1$ if $l$ is a tail-label. During training, the encoder $\phi_0(\cdot)$ remains frozen, and only the classifier parameters $W$ are fine-tuned.
        By adding $L_{\text{Aug}}$ to $L_{\text{BCE}}$, a more balanced loss is achieved, focusing on tail-labels without exacerbating the long-tail problem.
 Experimental results on three benchmark datasets (Eurlex-4K, Wiki10-31K,  AmazonCat-13K) demonstrate
 the effectiveness  of our proposed XDA method, particularly in
 improving the performance on tail-labels.


\paragraph{}
Dual-encoder (DE) models, effective in open-domain QA \cite{lee-etal-2019-latent}, are less explored in XMC. This paper \cite{gupta2024dualencoders} introduces novel DE modifications for XMC tasks. DE models, used in dense retrieval, map queries and documents into a shared embedding space for efficient fast similarity search \cite{johnson2017billionscale}. They excel with limited training data and single correct answers, using separate encoders for queries and documents. Existing  DE models underperform in XMC due to inappropriate training losses and the need for extensive parameters.
OvA-BCE does not train effectively and
InfoNCE \cite{oord2019representation} disincentivizes confident predictions. However, these losses
exhibit several limitations when applied to extreme multi-label
classification (XMC) tasks. Traditional contrastive losses like InfoNCE are suboptimal for multi-label settings as they enforce equal scoring for all positives, penalizing confident predictions.
To address these
limitations observed with the standard InfoNCE loss (XMC)
tasks, a re-formulation called DecoupledSoftmax loss, 
and a soft top-$k$ operator-based loss are proposed.

\paragraph{}
The decoupled softmax loss is defined as:
\[ l(q_i, y_i; s) = -\sum_{j \in [L]} y_{ij} \cdot \log \frac{e^{s(q_i, d_j)}}{e^{s(q_i, d_j)} + \sum_{l \in [L]} (1 - y_{il}) \cdot e^{s(q_i, d_l)}}, \]
where \( s(q_i, d_j) \) is the model-assigned score for the query-document pair \((q_i, d_j)\).
Here \( y_{ij} \) is 1 if document \( j \) is a positive label for query \( q_i \), and 0 otherwise.
This formulation removes positive label correlation in the denominator, improving training for DE models in XMC, provides more consistent and unbiased gradient feedback compared to standard softmax, essential for handling the imbalanced nature of XMC datasets.

\paragraph{}
Soft Top-$k$ Loss:
Designed to optimize prediction accuracy within a fixed budget size $k,$ particularly relevant for top-k predictions in XMC.
\begin{align*}
\ell(q_i, y_i; s) = - \frac{1}{L} \sum_{j \in [L]} y_{ij} \log z_{ij},
\end{align*}
where \( z_i = \text{SoftTop-}k(s_i) \) is the output of the soft top-$k$ operator applied to the score vector \( s_i = (s(q_i, d_1), \ldots, s(q_i, d_L)) \). The soft top-$k$ operator, taking a score vector as input, acts as a filter by assigning values near 1 to the top-$k$ scores and near 0 to the rest, ensuring differentiability for backpropagation.

\paragraph{}
The authors compared their DE approach to SOTA XMC methods like DEXA(Dual Encoder for eXtreme Classification Applications) \cite{inproceedings}, NGAME(Neural Graph Attention for Multi-label Extreme classification)\cite{dahiya2023ngame}, and XR-Transformer \cite{dahiya2021siamesexml}. Using the same distilbert-base model, their method outperformed these approaches on large-scale datasets (e.g., LF-Wikipedia-500K, LF-AmazonTitles-1.3M), achieving up to $2\%$  higher Precision@1 with $20\times$ fewer parameters.
The study shows that with the right loss formulation, DE models can achieve SOTA performance in XMC, offering parameter-efficient, generalizable solutions. Proper training losses help DE models overcome XMC's semantic gap. The study includes a memory-efficient, distributed implementation for large datasets using gradient caching \cite{gao-etal-2021-scaling}. 


\paragraph{}
The paper \cite{zhang-etal-2023-long} proposes a novel neural retrieval framework named DEPL (Dual Encoder with Pseudo
Label) for addressing the challenge of tail-label prediction in extreme multi-label text classification (XMTC). DEPL retrieval-based model leverages the semantic matching of document and label texts via a dual encoder model \cite{gao2021unsupervised} \cite{xiong2020approximate} \cite{luan2021sparse} \cite{karpukhin-etal-2020-dense},
which are generated automatically by a statistical model with BoW features. The primary goal is to enhance the mapping between input documents and system-enhanced label descriptions, thereby improving classification performance, particularly for rare labels.


%\textbf{Methodology:}
\paragraph{}
In the DEPL framework, a BoW classifier (SVM) is first trained to extract top keywords from label embeddings based on token importance. These keywords are concatenated with original label names to create pseudo descriptions. A BERT-based dense retrieval model \cite{devlin2019bert} is then used to rank labels by semantic matching between document text and these enhanced label descriptions. Pseudo labels generated this way improve the retrieval process.

%\textbf{Mathematical Background:}
\paragraph{}
The paper relies on the Johnson-Lindenstrauss (JL) lemma \cite{}from random matrix theory, which provides a mathematical foundation for connecting dense and sparse classifiers. This lemma helps establish a performance lower bound for the neural model under the assumption that neural embeddings behave similarly to random matrices.

%\textbf{Experiments and Results:}
\paragraph{}
The framework was extensively tested on large benchmark datasets, including EURLex-4K, AmazonCat-13K, Wiki10-31K and Wiki-500K. DEPL demonstrated significant improvements over strong baseline models, particularly in predicting tail labels. The experiments included ablation studies to understand the impact of pseudo label length on performance.

%\textbf{Limitations:}
\paragraph{}
The study acknowledges that the assumptions made for theoretical analysis may not hold in practical applications. Additionally, comparisons with other models and techniques, such as reranking losses and regularization, were not included in this work.



The paper \cite{10.1145/3539597.3570392} introduces NGAME, a novel method for negative mining in extreme classification (XC) that addresses the inefficiencies of existing techniques.  This approach allows for larger mini-batch sizes, faster convergence, and higher accuracy in training deep XC models, particularly when using large transformer-based encoders. \\

\paragraph{}
NGAME merges the tasks of mini-batch creation and negative mining, eliminating the need for a separate negative mining phase. This integrated approach results in mini-batches that naturally include informative negative samples, thereby accelerating the training process.
The method leverages in-batch sampling to provide high-quality hard negatives efficiently. During training, the method encourages data points and relevant labels to have similar embeddings. This similarity is used to distinguish between relevant and irrelevant labels. By using in-batch sampling, NGAME avoids the need for external structures or additional computations to find these negatives, thereby reducing memory and computational overheads. NGAME adapts the modular training pipeline from the DeepXML paper\cite{Dahiya_2021}. By reparameterizing label classifiers and leveraging label embeddings, the method enhances training efficiency and effectiveness.
NGAME’s algorithm clusters data point embeddings periodically and forms mini-batches from these clusters. Hard negatives are identified based on the proximity of label embeddings to data point embeddings.
The paper evaluates NGAME on multiple benchmark datasets from the Extreme Classification Repository, covering various applications such as product recommendation and Wikipedia page prediction. The method is compared against several baselines, including both Siamese (\cite{pmlr-v139-dahiya21a},\cite{10.1145/3437963.3441807},\cite{Mittal_2021}) and non-Siamese(\cite{jiang2021lightxml}, \cite{zhang2021fast},\cite{chang2020taming}) deep XC methods. The results demonstrate that NGAME achieves up to 16\% higher accuracy than state-of-the-art methods and shows significant improvements in click-through rates in live A/B tests on a popular search engine.

\paragraph{}
The paper \cite{10.1145/3580305.3599301} introduces DEXA, a framework addressing key limitations of existing encoder-based methods in Extreme Classification (XC). Models like NGAME(\cite{dahiya2022ngame}) and XR-Transformer(\cite{chang2020taming}) rely on embedding data points and labels into a shared space based solely on textual descriptions, which often fails in the presence of semantic gaps, especially in short-text applications. Modular training strategies used by these models train encoders independently of classifiers, resulting in suboptimal embeddings, particularly for underrepresented tail labels.\\
DEXA overcomes these issues by introducing auxiliary parameters shared across clusters of semantically related labels. These parameters act as correction terms, enriching label representations with latent information beyond text and reducing semantic distortions. By grouping labels into clusters using pre-trained embeddings and assigning shared auxiliary vectors, DEXA ensures representational adjustments for related labels, enhancing embedding quality. Integrating auxiliary parameters directly into encoder training eliminates the disjointed phases of methods like NGAME. Unlike XR-Transformer, DEXA achieves comparable or superior performance with a lightweight design, discarding auxiliary vectors after training to maintain efficiency.\\
DEXA demonstrates up to 6\% improvements in precision-based metrics and significant gains for tail labels on short-text datasets. On proprietary datasets like SponsoredSearch-40M, it achieves up to 15\% accuracy gains with smaller encoders, showcasing resource efficiency. It integrates seamlessly with encoders like DistilBERT and MiniLM, delivering consistent performance improvements without major architectural changes.


The paper \cite{Qaraei2024} addresses the challenge of training deep models for extreme multi-label classification (XMC) problems, where the output space can be extremely large. To address this issue the paper motivates the use of negative sampling and focuses on Maximum Inner Product Search (MIPS)  (\cite{auvolat2015clustering},\cite{8733051},\cite{shrivastava2014asymmetric})to identify hard negatives as an alternative to meta-classifier-based approaches(\cite{Dahiya_2021},\cite{jiang2021lightxml}), aiming to reduce computational overhead while maintaining or improving performance.\\
The paper highlights two significant issues in training deep models using MIPS-based negative sampling. Starting training with only hard negatives leads to high-magnitude gradients, causing large, unstable updates. Large intervals between MIPS pre-processing lead to non-informative negative samples, as the embeddings remain relatively unchanged, causing repetitive selection of the same negatives.\\
To mitigate the instability from using hard  negatives, the paper proposes a hybrid negative sampling approach. Select a few hard negatives using MIPS and combine them with negatives sampled from a uniform distribution. This balances the gradient magnitudes and stabilizes the training process.\\
To improve the efficiency of the MIPS process the authors use  a clustering-based approximate MIPS(\cite{auvolat2015clustering},\cite{8733051}). By clustering the label space, the search for hard negatives is restricted to a few representative clusters, reducing computational complexity while maintaining high-quality negative samples. By choosing an optimal number of clusters $(K = \sqrt{L})$, the method balances the computational load and the quality of the negatives retrieved, leading to a scalable and efficient training process.\\
Two architectures has been used as the encoders for the proposed method: a shallow neural network with a single 
hidden layer and a BERT model \cite{devlin2019bert} keeping its all the hyperparameters same as \cite{jiang2021lightxml}.
Experiments conducted on the Eurlex dataset, which includes approximately 4000 labels, validate the proposed methods.The hybrid method reaches performance levels comparable to state-of-the-art models like LightXML \cite{jiang2021lightxml}, without the additional overhead of training and storing a meta-classifier.


\paragraph{Comparison between methods}

\begin{itemize}
    \item XML-CNN although the first of the deep learning methods in XML, is no longer a competitive method in terms of performance. This is mainly because CNN's are not the best at capturing the information from text, and hence have been outperformed by most other methods.
    \item AttentionXML and XTransformer are both methods which require a lot of training time. However, they still remain relevant due to the fact that they perform significantly well on some datasets. In particular, AttentionXML performs well on datasets with high average feature text length.
    \item DeepXML based methods such as SiameseXML, ECLARE and NGAME are currently among the best performing methods in XML.
\end{itemize}

Over the last five years, deep learning based methods have outperformed all other methods in terms of performance. They have much higher accuracies than tree based methods, but can be slower in terms of train and test complexities and have higher model sizes.



==> DeepLearning/new-all-deep-learning-xml.tex <==
\paragraph{} Deep learning has surged in popularity over the past decade, becoming a dominant approach in many machine learning problems with abundant data. In extreme multi-label classification (XMC), however, deep learning methods emerged later due to several challenges. First, the extremely large output space (often thousands to millions of labels) means that a naïve deep model would require an enormous final layer and vast training resources. Second, the label distribution in XMC is highly imbalanced with a long tail of infrequent labels – for example, in the Wiki-500K dataset \cite{Bhatia16}, 98\% of labels have fewer than 100 training instances. This scarcity of data for most labels hinders deep models from learning reliable predictors for those tail labels. Early attempts to apply deep learning in XMC struggled with these issues, and for a time linear methods and tree-based methods dominated the field. Nevertheless, deep learning excels at extracting context-dependent features from raw text via nonlinear representations. This ability to learn rich text embeddings challenged the traditional bag-of-words representations in XMC and paved the way for deep learning-based methods to gain traction. 

\paragraph{} The first notable deep learning approach for XMC was XML-CNN proposed by Liu et al. (2017) \cite{liu2017deep}. This method adapted the successes of deep learning in multi-class text classification – such as FastText \cite{joulin2016bag}, CNN-based sentence classifiers \cite{chen2015convolutional}, and a bag-of-words CNN variant \cite{liu2017deep} – to the extreme multi-label setting. XML-CNN employs a family of convolutional neural networks (CNNs) to encode input text into a compact representation, and was among the earliest to demonstrate the feasibility of deep learning for XMC. Its architecture (illustrated in Fig.~\ref{fig:CnnXML}) combines ideas from prior CNN models: using multiple convolution filters of various sizes (as in Kim’s CNN~\cite{kim2014}), applying a dynamic max-pooling layer (as in the Bow-CNN~\cite{johnson2015effectiveusewordorder}, adapts bag of words to convolution) to better capture informative $n$-grams from different parts of the document, a bottleneck fully-connected layer to reduce dimensionality, and a sigmoid output layer with binary cross-entropy loss for multi-label prediction. In effect, the network learns to project each document into a low-dimensional latent space and then predicts relevant labels in one pass.
By using a bottleneck layer, the number of parameters in the final layer is dramatically reduced (from $t p \times L$ to $h \times (t p + L)$, where $L$ is number of labels, $t$ number of filters, $p$ pooling segments, $h$ bottleneck size), making the model more memory-efficient. XML-CNN was an important proof-of-concept, showing that deep networks can outperform traditional methods by learning context-aware features. However, a single CNN encoder has limited ability to focus on the most relevant parts of the text for each specific label. This drawback meant that while XML-CNN improved general performance, it sometimes failed to capture fine-grained label-specific cues in the input, leaving room for improvement by more sophisticated architectures. 
%
\begin{figure}[t!] 
\centering 
\includegraphics[scale=0.4]{Images_K/XML_CNN.drawio.png} 
\caption{\label{fig:CnnXML} The XML-CNN model } 
\end{figure} 
%
Finally, the output of the bottleneck layer is passed through another fully connected layer with output size $L$. The binary cross entropy loss is applied over the sigmoid outputs for training. \paragraph{} Building on these ideas, You et al. (2019) introduced AttentionXML \cite{you2019attentionxml}, which incorporates an attention mechanism to better identify the parts of each input text that are most relevant to each label. The model uses a Bidirectional LSTM encoder to capture long-range word dependencies, and a multi-label attention module that produces label-specific document representations. In essence, for each potential label, the attention mechanism learns a weight distribution over the words in the document, allowing the model to focus on label-indicative words or phrases. To manage the huge label space, AttentionXML employs a shallow and wide probabilistic label tree (PLT) structure over labels. The deep model (BiLSTM with multi-head attention) is applied at each node of this label tree, which decomposes the problem into predicting a path of label clusters and eventually leaf labels. Figure \ref{fig:AttnXML} illustrates the attention-aware architecture of this model. By combining label tree-driven reduction with per-label attention, AttentionXML achieved significantly higher Precision@1 than XML-CNN and other contemporaries, and its propensity-scored metrics showed strong performance even on tail labels. The ablation studies in \cite{you2019attentionxml} confirmed that the multi-head attention was crucial for these gains. The trade-off, however, is computational: training and inference with AttentionXML are resource-intensive due to the need to train a BiLSTM+attention model for every node in the label tree. This made AttentionXML slow to train and deploy, especially on datasets with millions of labels. Its success nevertheless demonstrated that attention-based sequence models can substantially improve extreme classification, especially for datasets with longer text inputs (where the ability to attend to relevant words is most beneficial). This insight set the stage for transformer-based models, which use self-attention to encode text more efficiently. 

\begin{figure}[t!] \centering \includegraphics[scale=0.3]{Images_K/AttentionXML.drawio.png} \caption{\label{fig:AttnXML} An Illustration of Attention Aware Deep Model in AttentionXML } \end{figure} 

\paragraph{} Despite the effectiveness of AttentionXML’s label-wise attention, its heavy architecture motivated researchers to explore pretrained Transformers for XMC, hoping to leverage models like BERT \cite{devlin2019bert} that had revolutionized many NLP tasks. A direct application of transformers to XMC (treating it as a very large multi-label classification task) naively would require extremely large output layers and memory, resulting in subpar performance and out-of-memory issues. To overcome this, Chang et al. (2020) proposed X-Transformer \cite{chang2020taming}, which tames the large label space by breaking the task into manageable subtasks using label clustering. In X-Transformer, the labels are first clustered (using semantic label text embeddings) into a moderate number of meta-labels. This forms a two-level hierarchy: each cluster can be treated as a pseudo-label representing a set of original labels. The model then has three components: (1) a Label Clusterer that groups labels into, say, $K$ clusters using algorithms like balanced $k$-means, (2) a Transformer-based Matcher that is fine-tuned to predict which label clusters are relevant for a given input, and (3) a final Ranker that, for each input, considers only the small subset of labels in the predicted clusters and ranks these labels by relevance. During the matching stage, each training instance is only associated with its cluster(s) of true labels, drastically reducing the effective output space for the transformer. At inference, given a new text, the transformer encoder (fine-tuned for matching) produces an embedding used to pick a few most likely label clusters, and then only labels from those clusters are scored (often with a simpler model or another round of fine-tuning within the cluster). By sequentially narrowing down the label candidates, X-Transformer manages to scale transformer fine-tuning to extremely large $L$. Empirically, it performed well across various public XMC benchmarks, and at the time was outperformed only by AttentionXML on certain datasets. Soon after, Ye et al. (2020) presented APLC-XLNet \cite{ye2020pretrained}, which similarly leveraged the XLNet transformer model \cite{yang2019xlnet} for XMC. APLC-XLNet stands for Adaptive Probabilistic Label Clusters with XLNet. Like X-Transformer, it avoids training on the full label set directly by using a data-driven clustering of labels (the adaptive probabilistic label clustering) and then fine-tuning XLNet on those clusters. These early transformer-based approaches demonstrated that with careful partitioning of the label space, one can harness powerful pretrained language models for extreme classification. 

\paragraph{} Subsequent research addressed some limitations of these transformer-based frameworks. One issue in methods like AttentionXML or the original X-Transformer was the use of a static negative sampling strategy: each training instance would repeatedly see the same sampled negative labels (non-relevant labels), which could lead to overfitting to that particular set and suboptimal generalization. Jiang et al. (2021) tackled this with LightXML \cite{jiang2021lightxml}, which introduces dynamic negative sampling in a generator–discriminator setup. LightXML’s architecture fine-tunes a Transformer (e.g., BERT) in two parts: a generator module first recalls a shortlist of candidate labels for each input (akin to a preliminary retrieval of possibly relevant labels), and then a discriminator module ranks these candidates, refining the predictions. Crucially, the generator’s shortlists are updated throughout training rather than being fixed beforehand. This means the model is continually exposed to new ``hard'' negatives (labels that are likely but not actually relevant), forcing it to remain robust and not simply memorize a small negative set. This dynamic interplay keeps training challenging and was shown to improve accuracy over static sampling methods. Around the same time, Zhang et al. (2021) introduced XR-Transformer \cite{zhang2021fast}, which further improved the efficiency of transformer models on extreme scales. XR-Transformer uses a recursive hierarchical labeling approach: it builds a hierarchy of labels using balanced $k$-means clustering (producing a tree of label clusters) and then recursively fine-tunes a transformer on increasingly narrower subsets of labels. At the root level, the model sees all data but with very coarsely grouped labels; at deeper levels, it handles fewer labels and can fine-tune more discriminatively. During inference, XR-Transformer traverses the label tree: at each level, it uses the learned transformer to pick which branch (cluster) the input should follow, thereby exponentially cutting down the number of labels considered. An interesting innovation in XR-Transformer is the combination of sparse and dense features: it augments the transformer's text embedding with TF-IDF features of the input, to compensate for any information lost due to the transformer's input length limit or semantic biases. This hybrid representation leverages the strength of statistical features (which can capture keyword matches even for very rare terms or substrings) alongside deep contextual embeddings. Thanks to these techniques, XR-Transformer achieved notable gains in both training speed and accuracy on large benchmarks – for instance, on the Amazon-3M dataset (with about 3 million labels), XR-Transformer improved Precision@1 from ~51.2\% to ~54.0\% while reducing training time from 23 hours to just 3.5 hours, a huge efficiency boost. 

\paragraph{} Beyond architectural improvements, another trend in deep XMC has been label-aware learning, i.e. leveraging label metadata or correlations within the model. Many deep methods traditionally treated labels as abstract indices, only learning a classifier weight or embedding for each through supervision. Newer approaches instead utilize the information in label descriptions or label co-occurrence graphs to improve performance, especially for tail labels. GalaXC (Saini et al., 2021) \cite{saini2021galaxc} is one such example that uses a graph neural network to jointly embed documents and labels. In GalaXC, a graph is constructed where each document and each label is a node, and edges connect documents to the labels they have (and possibly labels to other labels that co-occur). Graph convolution layers (with attention) propagate information in this document–label network, so that the representation of a label node can be influenced by other related labels and the documents they appear in. By performing multiple graph hops, GalaXC effectively shares context among related labels and between labels and documents, which helps especially in cases where a label has very few training examples (its representation can still be enriched via connected labels or documents). A related method, ECLARE (Mittal et al., 2021) \cite{mittal2021eclare}, also incorporates label metadata and label correlations into a deep framework. ECLARE extends the DeepXML pipeline (discussed below) by utilizing label textual descriptions and a label correlation matrix to influence the learning process. By attending to label features, these models become more label-aware, meaning the model’s representation of an input can be modulated by knowledge of the candidate labels themselves. Such techniques tend to particularly help with tail labels (labels with few samples), since even if a tail label has little direct data, the model can infer its relevance via similarity to other labels or via its description. 

\paragraph{} A general observation in XMC is that training a deep model on the full label set is often intractable, so most high-performing methods employ some form of two-stage or modular training. This was formalized by Dahiya et al. (2021) in the DeepXML framework \cite{Dahiya_2021}, which many recent methods follow. The DeepXML framework breaks the problem into four modules, each designed to be scalable. (i) In the first module, an intermediate representation of documents is learned by training on a surrogate label set – typically a smaller set of labels that are representative of the whole label space (for example, the set of head labels that have plenty of data, or a set of label clusters). This gives an initial text encoder that is already good at separating some labels. (ii) The second module performs label shortlisting or negative sampling: for each training instance, instead of considering all $L$ labels as negative, it selects a subset $N_i$ of “hard” negative labels that are most confusable with the true labels. These are often chosen by nearest-neighbor search in the learned embedding space (or by clustering or hashing techniques) so that each instance only needs to confront $O(\log L)$ negative labels per update. (iii) The third module uses transfer learning to refine the encoder on the full label set: the encoder (and possibly classifier) from module (i) can be fine-tuned on the tail labels or the remaining data, effectively transferring knowledge from the easier surrogate task to the full XMC task. (iv) The final module makes the predictions, often using an efficient indexing structure (like an approximate nearest neighbor search, ANNS, or a classifier chain) to retrieve the top labels for each input without scoring every label. Many of the best recent deep XMC methods can be viewed as instantiations of this DeepXML pipeline. For example, ASTEC (Dahiya et al., 2021) \cite{dahiya2021deepxml} is a method that explicitly uses this framework: it clusters labels to create the surrogate label set in module (i), uses an ANNS structure for hard-negative mining in module (ii), and fine-tunes a transformer encoder for the final predictions. ASTEC achieved state-of-the-art results on several datasets, demonstrating the effectiveness of the modular approach. 

\paragraph{} Another prominent DeepXML-based method is SiameseXML (Dahiya et al., 2021) \cite{dahiya2021siamesexml}, which learns a joint embedding space for instances and labels using Siamese networks. The goal is to embed each document and each label into the same vector space such that a document embedding is close to those of its relevant labels and far from those of irrelevant labels. To train this, SiameseXML uses a contrastive loss (such as a triplet loss or pairwise hinge loss) and performs hard negative mining – selecting particularly challenging negative labels for each positive instance–label pair to include in the loss. By doing so, the model focuses on separating each instance from the “closest” wrong labels. SiameseXML also makes use of label text features (e.g., product titles or category names as label representations) to initialize or assist the label embeddings, which helps inject semantic knowledge of labels. The Siamese setup naturally fits into the DeepXML paradigm: after learning the joint embeddings on a representative set of labels and mining hard negatives, at inference time one can use a fast similarity search (ANNS) to find the nearest label embeddings to a given document’s embedding, rather than computing a full classifier matrix multiplication. This makes prediction extremely efficient and scalable to very large $L$. SiameseXML was shown to outperform earlier methods like AttentionXML and X-Transformer on large-scale datasets, establishing that embedding-based retrieval can be a powerful approach in XMC. \paragraph{} A recent extension of this embedding-based approach is NGAME (Neural Graph Attention for Multi-label Extreme Classification) \cite{dahiya2023ngame}. NGAME’s primary innovation is in how it constructs training batches to perform implicit negative sampling. In standard Siamese or metric learning approaches, if we take random batches of instances, the set of labels present in the batch serves as negatives for each other instance. But random batches might contain mostly unrelated instances with completely disjoint labels, yielding trivial negatives. NGAME instead clusters the training instances periodically and forms mini-batches with similar instances. Consequently, the labels that appear in a given mini-batch are likely to be relevant to at least one of the batch’s instances and act as more informative negatives for the other instances. In effect, NGAME merges the negative mining step with the batching process: by training on clusters of related examples, each instance in a batch is confronted with hard negatives (labels that are semantically close or confusable) without an explicit mining algorithm. This approach allowed the use of larger batch sizes (since each batch is more label-homogeneous, the combined label set doesn’t blow up as quickly), which stabilized training and led to faster convergence. Empirical evaluations showed that NGAME could accelerate training by avoiding separate negative mining passes, and it achieved up to 16\% higher accuracy than prior state-of-the-art methods on certain extreme classification benchmarks. Impressively, NGAME also demonstrated real-world impact by improving click-through rates in live search engine A/B tests, indicating that the better negative sampling strategy translated to more relevant predictions in practice. NGAME’s success underscored the importance of effectively handling negatives in extreme classification, further corroborated by other research focused on this aspect. 

\paragraph{} While SiameseXML and NGAME focus on learning from text descriptions alone, one limitation of embedding-only methods is the semantic gap: if two labels have similar meanings but different wording (or if a label’s name doesn’t fully convey its meaning), a text-based encoder might embed them poorly. Chandak et al. (2023) address this with DEXA (Dual Encoder for eXtreme Applications) \cite{10.1145/3580305.3599301}. DEXA augments the label representations with learned auxiliary vectors that are shared among clusters of semantically related labels. In practice, labels are first grouped (using pre-trained embedding similarity or co-occurrence) into a number of clusters. Each cluster is given an auxiliary trainable embedding, and each label representation is the sum of the transformer-encoded label text and a fraction of these auxiliary vectors (for clusters it belongs to). These auxiliary parameters act as correction terms that can capture aspects of label meaning not evident from the raw text alone, thereby reducing semantic distortions. During training, DEXA jointly learns the text encoder and these auxiliary label vectors in an end-to-end fashion, integrating what would otherwise be an external label clustering or augmentation step into the model itself. This is unlike methods such as NGAME or XR-Transformer which have distinct phases (embedding learning, then clustering or matching); DEXA’s training is a single cohesive process. After training, the auxiliary vectors can be removed, so at inference time DEXA behaves like a standard dual encoder (document encoder and label encoder) without extra overhead. DEXA delivered significant accuracy improvements, particularly on datasets with very short text inputs (where label semantics are harder to discern): it boosted precision-based metrics by up to 6\% and noticeably improved tail-label prediction. On a massive industrial dataset (SponsoredSearch-40M, with tens of millions of labels), DEXA achieved up to 15\% higher accuracy using smaller transformers (like DistilBERT, MiniLM), highlighting its ability to improve performance and efficiency at scale. These gains illustrate how enriching label representations via learned meta-parameters can help bridge the gap between label text and label meaning in extreme classification. 

\paragraph{} A complementary direction to improving architectures is to optimize the training process itself for extreme scale. Negative sampling is one such focus area. As mentioned, methods like LightXML and NGAME work hard to present useful negative examples to the model. Qaraei et al. (2024) specifically examine negative sampling for deep XMC and propose a novel strategy to address its pitfalls \cite{Qaraei2024}. They advocate using Maximum Inner Product Search (MIPS) to find hard negatives on the fly during training. In each iteration, given the current document embedding (from a deep encoder) and all label embeddings, a MIPS query can retrieve labels that have the highest predicted similarity to the document but are not actually correct labels – these are intuitively the “hardest” negatives because the model currently mistakes them as likely positives. However, the authors identified two issues when naively using only MIPS-hard negatives: (1) Instability in early training – if the model is presented with only very hard negatives from the start, the loss gradients tend to be large (since the model is very wrong about these negatives initially), leading to extreme updates that can destabilize training. (2) Staleness of negatives – performing MIPS search infrequently (e.g., every few epochs) means the label embeddings used for MIPS become outdated as the model learns, and it might keep selecting the same negatives repeatedly even after they cease being informative. To solve the first issue, Qaraei et al. propose a hybrid negative sampling approach: mix a few MIPS-selected hard negatives with some randomly sampled negatives in each batch. The random negatives (usually easy ones) keep gradient magnitudes in check, while the hard negatives ensure the model is challenged – this balance yields more stable updates. To address the second issue of stale negatives, they make the negative mining more efficient so it can be done more frequently. They use a clustering-based approximate MIPS technique: the label embeddings are periodically clustered into $\sqrt{L}$ clusters, and for a given document embedding, MIPS is performed only within the top few nearest clusters rather than the entire label set. This significantly cuts down the search time (a classic speedup in high-dimensional search tasks), allowing them to refresh the hard negatives more often during training. The result is a scalable training procedure that yields high-quality negatives throughout learning. They demonstrated this method on the Eurlex-4K dataset (a legal document dataset with around 4K labels) using two encoder architectures – a simple single-hidden-layer feed-forward network and a BERT-based encoder (with hyperparameters similar to LightXML’s). In both cases, the hybrid negative sampling method reached performance comparable to state-of-the-art models like LightXML, without needing the complex two-module structure or additional meta-classifiers that some deep XMC models use. This work highlights that smart training tricks can mitigate computational overhead even when using powerful deep encoders on extreme label sets. 

\paragraph{} In addition to these major methodologies, there have been other innovative approaches targeting specific challenges in XMC. One such challenge is the extreme imbalance between head labels and tail labels. BoostXML (2022) \cite{chu2022boostxml} is a method designed explicitly to improve tail-label prediction by integrating gradient boosting ideas into a deep neural network. It observes that most deep XMC models tend to optimize for overall accuracy (dominated by head labels), so BoostXML introduces a two-stage training process to emphasize tail performance. In the first stage, it trains a deep model (similar to AttentionXML’s BiLSTM+attention backbone) end-to-end on the data using a standard binary cross-entropy loss, obtaining a strong base encoder. In the second stage – the boosting stage – BoostXML keeps the encoder fixed and sequentially trains a series of small weak learners (e.g., small multi-layer perceptrons) that focus on the residual errors of the current model. Each new weak learner is trained on the residual (the difference between the true label vector and the current model’s prediction) and is weighted (with a scaling factor $\rho_t$) before being added to the model’s prediction ensemble. By using both first-order and second-order gradient information, the boosting step particularly amplifies the learning on labels that were mispredicted (often the tail labels). After adding a new weak learner, a corrective step fine-tunes the entire network (encoder + all learners) briefly with a small learning rate using the standard loss to adjust for any overshooting. This process repeats for a number of boosting rounds. The outcome is an ensemble deep model that has explicitly corrected its mistakes on tail labels through multiple iterations, without significantly degrading head label performance. Experiments on several benchmark datasets showed that BoostXML can indeed outperform prior state-of-the-art, with especially large gains on tail label metrics, while maintaining competitive performance on head labels. 

\paragraph{} Another noteworthy approach is MatchXML (2022)~\cite{matchxml}, which reformulates multi-label classification as a text–label matching problem. Instead of directly outputting label scores from a single network, MatchXML fine-tunes a transformer by feeding it pairs of <document, label> and training it to output a high similarity for true pairs and low for random pairs. In practice, each mini-batch consists of a set of documents and a sampled set of labels (some relevant, some not for each document); the transformer encoder (with a special text+label input format) is trained with a contrastive objective to distinguish matching pairs from mismatches. This approach effectively learns an embedding where documents and labels that are related have high inner product. MatchXML also incorporates static label embeddings from pre-trained Sentence-BERT and sparse TF-IDF features for labels, which are kept fixed, alongside the fine-tuned transformer embeddings. By leveraging both fixed and fine-tuned representations, it captures both general semantic relatedness and task-specific alignment. An ablation study showed that this combination (coarse static embeddings + fine-tuned matching) improved performance across various datasets. MatchXML reported superior accuracy and faster training compared to many existing methods, showcasing a viable alternative training paradigm for XMC. 

\paragraph{} We see that deep learning-based XMC methods have diversified into various architectural and algorithmic innovations: convolutional encoders, recurrent networks with attention, transformer models with label clustering, graph neural networks for label graphs, Siamese dual-encoders with metric learning, boosted ensembles, and beyond. Table \ref{tab:deep_methods_comp} (hypothetical reference) could summarize their key features. To put things in perspective, we highlight a few overarching comparisons: 

\begin{itemize} 

\item XML-CNN (CNN-based) was a pioneering deep approach but is no longer competitive in accuracy. CNNs (without attention) struggle to capture the full context of the text, so later models that use attention or transformers have largely outperformed XML-CNN. 

\item AttentionXML and X-Transformer (early attention and transformer models) achieve high accuracy, but often at the cost of very large training times and model complexity. They remain relevant for certain applications; for example, AttentionXML excels on datasets with long documents, where its label-wise attention can fully exploit the rich text. X-Transformer and similar transformer-based methods set strong baselines but needed subsequent efficiency improvements. 

\item LightXML and XR-Transformer improved transformer-based XMC by introducing dynamic negative sampling and recursive fine-tuning, respectively, substantially reducing training time while maintaining state-of-the-art accuracy. These highlight the importance of hierarchical label structures and online hard negative mining in scaling deep models. 

\item DeepXML-based methods such as SiameseXML, ECLARE, and NGAME (and others like ASTEC and DEXA) are among the current best performers in XMC. They leverage label text features, joint embedding spaces, and advanced negative sampling or label augmentation techniques to push the envelope in prediction accuracy. Many of them specifically tackle the tail-label challenge and achieve a better balance between head and tail prediction than earlier methods. 

\end{itemize} 

Over the last five years, deep learning-based methods have indisputably outperformed earlier approaches in terms of accuracy on extreme classification benchmarks. They deliver significantly higher precision and recall than traditional tree-based or one-vs-all methods. The gains come from their ability to learn powerful representations and capture label dependencies, but these models are also typically slower to train and evaluate, and often require larger model sizes. Thus, a recurring theme in recent research is improving scalability – through smarter training (negative sampling, clustering, curriculum learning) and efficient architectures – so that the superior accuracy of deep models can be attained without prohibitive computational cost.

==> LinearAlgebra/Submodular.tex <==
\subsection{A Submodular Feature-Aware Framework for Label Subset Selection in Extreme Classification}

This paper tackles three important inherent problems arising extreme multi-label classification:

\subsubsection{Label Space Transformation}
\begin{itemize}
    \item Transforming problem to a small tractable space.
    \item Making the problem more complicated by transforming to a new non-sparse space.
    \item Information loss caused by projecting to low dimension.
    \item Using assumptions like low-rank, incompatible with real data.
    
    
      \begin{figure}[H]
        \centering
        \includegraphics[width=80mm]{Images_SK/submodular_1.PNG}
        \caption{Label space transformation}
    \end{figure}{}
    
\end{itemize}

\subsubsection{Label Space Partitioning}
\begin{itemize}
    \item Avoid information loss caused by dimension reduction.
    \item Using expensive optimization methods to partition the samples at each node, which is a very complicated and unstable problem for high-dimensional spaces.
    \item Using an ensemble of the learners in order to overcome the instability and improve prediction accuracy.
\end{itemize}

\subsubsection{Label Subset Selection}
\begin{itemize}
    \item Strong mathematical error bounds.
    \item Expensive methods for subset selection. 
    \item Prediction Error propagates from selected subset through remaining labels.
    \item Ignoring the labels less dependent to the other labels.
\end{itemize}

In this paper, the issues stated above in the 3rd group: Label Subset Selection is addressed. The approach proposed to solve these issues also indirectly solve the problems arising in group 1 and 2 are as follows:

\begin{itemize}
    \item Avoiding transformation and information loss of 1st group.
    \item No need of an ensemble to avoid suffering from instability of 2nd group.
    \item Considering training error and avoiding expensive selection methods of 3rd group and ensuring that it is feature aware.
    
\end{itemize}

\subsubsection{Submodular Subset Scoring Function}
The main idea of the paper is based on landmark selection framework for selecting the most informative labels \& to solve the multi-label learning problem with these labels. Submodular maximization framework with linear cost to find informative labels which are most relevant to the other labels yet least redundant with each other. It can be better understood with graph based analogy as shown below:

 \begin{figure}[H]
        \centering
        \includegraphics[width=100mm]{Images_SK/submodular_2.PNG}
        \caption{Graph of Label Relationship}
    \end{figure}{}

Framework includes both label-label and label-feature dependencies, which aims to find the labels with the most representation and prediction ability. In contrast to the other similar approaches, it also considers label-feature dependencies and outlier labels that are highly independent of other labels as depicted below by considering both edge thickness and node thickness.

\begin{figure}[H]
        \centering
        \includegraphics[width=100mm]{Images_SK/submodular_3.PNG}
        \caption{Graph of Label-Feature Relationship}
    \end{figure}{}

Solving the problem using the selected (smaller number of) labels leads to minimizing both representation and training error. Representation ability is equivalent to the power of the selected subset to reconstruct the remaining labels. Prediction ability is equivalent to training accuracy leading to less error propagation from predicted label subset to the remaining labels during reconstruction. The tree based approaches suffer from error propagation through the hierarchy and need many training samples to avoid under-fitting in the lower levels of the partitioning tree.

\subsubsection{Landmark Information Propagation}
The main step of our proposed framework is to propagate the predicted value for the selected label subset to the full set of labels in order to recover the original space.
A linear dependency between the selected labels $Y_{s}$ and the full set of labels $Y$ by a matrix $Z$ and the extracting the outlier labels as matrix $E$. This linear propagation is achieved using ADMM optimization algorithm.

\begin{figure}[H]
        \centering
        \includegraphics[width=100mm]{Images_SK/submodular_4.PNG}
        \caption{Landmark Information Propagation}
    \end{figure}{}

In the prediction step, this linear function obtains the full label set by combining the subset $(Y_{s})$ and outlier predictions $(E)$ predicted by the regression functions.
